Indoor Localization for an Autonomous Model Car: A Marker-Based Multi-Sensor Fusion Framework

Global navigation satellite systems readily provide accurate position information when localizing a robot outdoors. However, an analogous standard solution does not exist yet for mobile robots operating indoors. This paper presents an integrated framework for indoor localization and experimental validation of an autonomous driving system based on an advanced driver-assistance system (ADAS) model car. The global pose of the model car is obtained by fusing information from fiducial markers, inertial sensors and wheel odometry. In order to achieve robust localization, we investigate and compare two extensions to the Extended Kalman Filter; first with adaptive noise tuning and second with Chi-squared test for measurement outlier detection. An efficient and low-cost ground truth measurement method using a single LiDAR sensor is also proposed to validate the results. The performance of the localization algorithms is tested on a complete autonomous driving system with trajectory planning and model predictive control.

==> sections/subsections/trajectory_planning.tex <==
\subsection{Trajectory Planning and control}
% Xibo
In an autonomous driving scenario, the pose determined by the indoor localization algorithm forms an input to the motion planning and control modules of the mobile robot. 
In order to evaluate the positioning performance of various localization algorithms, the entire planning and control methods are also implemented. For motion planning, the well-known hybrid state A\uppercase{*} algorithm is adapted with three improvements \cite{folkers2020time}:
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/trajectory_planning.png}
	\caption{Trajectory generated by the motion planning. The trajectory and free-space polygon are
		displayed in orange and green respectively. The black line segment in the middle of the lane represents the voronoi edges
		of a voronoi diagram}
	\label{fig:trajectory_planning}
\end{figure}

\textbf{Free-space Polygon}: we generated a free-space polygon through the route planning module. As shown in Figure \ref{fig:trajectory_planning}, the green free-space polygon restricts the accessible area of the miniature vehicle. Lane information inside the free-space polygon area is considered. After determining the area of free-space polygon, the planning trajectory will be generated based on the voronoi field.


\textbf{Voronoi field}: similar to \cite{dolgov2010path}, the voronoi field is used to compute the reference path inside the free-space polygon. A feasible trajectory is generated by considering the static and moving obstacles. In this paper, we only presented the trajectory through the middle of the lane, which is used as a reference trajectory for the controller.  

\textbf{Kinematic vehicle model}: as the hybrid state A\uppercase{*} algorithm, the kinematic requirements of the vehicle is also considered in our motion planning. The feasible trajectory is generated according to our single-track model presented in Eq.\ref{eq:system-model}. The entire trajectory with the time series is taken as the input of the model predictive controller. 

In order to fulfill various driving scenarios in the autonomous driving, the trajectory is generated in every 100 ms. Therefore, not like normal trajectory tracking, the controller in our case must be able to handle a dynamic trajectory input with 100 ms input frequency. For each reference trajectory, the controller formulate it as a optimal control problem (OCP). 
\begin{align}
\begin{split}
\min_{s,u,T} \quad &J(s,u,T)\\
\text{s.t. } \dot{s}(t) &= f(s(t),u(t)),\\
s_\text{min} &\leq s(t) \leq s_\text{max},\\
u_\text{min} &\leq u(t) \leq u_\text{max},\\
\varPsi(s(0),s(T)) &= 0,\\
C(s(t),u(t),t) &\leq 0 \text{ for all } t \in [0,T],
\end{split}
\label{eq:ocp}
\tag{OCP}
\end{align}
where the $J$ represents the objective function. The control output $u$ is generated according to the giving states $s$, the nonlinear dynamic function $f$, the initial condition $\varPsi$ and the general path constrains $C$. For more details of the MPC controller can be referred to \cite{rick2019autonomous}.

